Per-Gaussian Embedding-Based Deformation for Deformable 3D Gaussian Splatting

As 3D Gaussian Splatting (3DGS) provides fast and high-quality novel view synthesis, it is a natural extension to deform a canonical 3DGS to multiple frames for representing a dynamic scene. However, previous works fail to accurately reconstruct complex dynamic scenes. We attribute the failure to the design of the deformation field, which is built as a coordinate-based function. This approach is problematic because 3DGS is a mixture of multiple fields centered at the Gaussians, not just a single coordinate-based framework. To resolve this problem, we define the deformation as a function of per-Gaussian embeddings and temporal embeddings. Moreover, we decompose deformations as coarse and fine deformations to model slow and fast movements, respectively. Also, we introduce a local smoothness regularization for per-Gaussian embedding to improve the details in dynamic regions. Project page: https://jeongminb.github.io/e-d3dgs/

==> tabs/project_page.tex <==
% \FloatBarrier
\begin{table}[H] 
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc}
\multicolumn{1}{l|}{\multirow{2}{*}{\diagbox[]{Model}{Dataset}}} & \multicolumn{3}{c|}{\textbf{Neural 3D Video}}
& \multicolumn{3}{c|}{\textbf{Technicolor Light Field}} 
& \multicolumn{3}{c}{\textbf{HyperNeRF}}    
\\ \cline{2-10}  
& PSNR$\uparrow$ & {SSIM$\uparrow$} & {LIPIPS$\downarrow$}  
& PSNR$\uparrow$ & {SSIM$\uparrow$} & {LIPIPS$\downarrow$}
& PSNR$\uparrow$ & {SSIM$\uparrow$} & {LIPIPS$\downarrow$}
\\ \hline

\multicolumn{1}{l|}{D3DGS}                                        & - & -& -& -& -& - & 22.40 & 0.598 & 0.275 \\

\multicolumn{1}{l|}{4DGaussians}                                  & 30.71 & 0.935 & 0.056 & 29.62 & 0.844 & 0.176 & 25.03 & 0.682 & 0.281 \\ 

\multicolumn{1}{l|}{\textbf{Ours}} 
& \textbf{31.31} & \textbf{0.945}& \textbf{0.037}& \textbf{33.24}& \textbf{0.907}& \textbf{0.100}& \textbf{25.43}& \textbf{0.697}& \textbf{0.231}  \\                               
\end{tabular}
}
\end{table}

